Spatial Imagination With Semantic Cognition for Mobile Robots

The imagination of the surrounding environment based on experience and semantic cognition has great potential to extend the limited observations and provide more information for mapping, collision avoidance, and path planning. This paper provides a training-based algorithm for mobile robots to perform spatial imagination based on semantic cognition and evaluates the proposed method for the mapping task. We utilize a photo-realistic simulation environment, Habitat, for training and evaluation. The trained model is composed of Resent-18 as encoder and Unet as the backbone. We demonstrate that the algorithm can perform imagination for unseen parts of the object universally, by recalling the images and experience and compare our approach with traditional semantic mapping methods. It is found that our approach will improve the efficiency and accuracy of semantic mapping.

==> content/acknowledgment.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex



==> content/keywords.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex


%\begin{IEEEkeywords}
%	Virtual Reality and Interfaces, Localization, Object Detection, Computer Vision for Other %Robotic Applications, AI-Based Methods
%\end{IEEEkeywords}

==> content/title.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex

%\title{A robust pose estimator for articualted robots using monocular cameras and Deep-Learning-based keypoint detection\\
%	}
%	\thanks{Identify applicable funding agency here. If none, delete this.}
%}
\title{\LARGE \bf
Towards Augmented Reality Simulation in Robotics - Facing Barriers of Industrial Applicability
}

\author{Jens Lambrecht$^{1}$, Linh Kästner$^{1}$, Jan Guhl$^{2}$ and J\"org Kr\"uger$^{2}$% <-this % stops a space% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Jens Lambrecht and Linh Kästner are with the Chair Industry Grade Networks and Clouds, Faculty of Electrical Engineering and Computer Science,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small lambrecht@tu-berlin.de}}%
\thanks{$^{2}$Jan Guhl and J\"org Kr\"uger are with the Chair Industrial Automation Technology, Faculty of Mechanical Engineering and Transport Systems,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small guhl@iat.tu-berlin.de}}%        
}


%\author{
%	\IEEEauthorblockN{Jens Lambrecht}
%	\IEEEauthorblockA{\textit{Chair Industry Grade Networks and Clouds} \\
%		\textit{Technische Universität Berlin}\\
%		Berlin, Germany \\
%		lambrecht@tu-berlin.de}
%}

\maketitle
